Improved Gradient based Adversarial Attacks for Quantized Networks

Neural network quantization has become increasingly popular due to efficient memory consumption and faster computation resulting from bitwise operations on the quantized networks. Even though they exhibit excellent generalization capabilities, their robustness properties are not well-understood. In this work, we systematically study the robustness of quantized networks against gradient based adversarial attacks and demonstrate that these quantized models suffer from gradient vanishing issues and show a fake sense of robustness. By attributing gradient vanishing to poor forward-backward signal propagation in the trained network, we introduce a simple temperature scaling approach to mitigate this issue while preserving the decision boundary. Despite being a simple modification to existing gradient based adversarial attacks, experiments on multiple image classification datasets with multiple network architectures demonstrate that our temperature scaled attacks obtain near-perfect success rate on quantized networks while outperforming original attacks on adversarially trained models as well as floating-point networks. Code is available at https://github.com/kartikgupta-at-anu/attack-bnn.

==> tables/apgd_square.tex <==
\begin{table}[]
\centering
\small
\begin{tabular}{l|cccc|cccc}
\toprule[1.5pt]
 \multirow{3}{*}{\textbf{Method}} & \multicolumn{4}{c|}{\textbf{\sresnet{-18}}} & \multicolumn{4}{c}{\textbf{\svgg{-16}}} \\
 \cmidrule[1pt]{2-9}
 & \multirow{2}{*}{\textbf{\acrshort{APGD}}} & \textbf{Square} & \multicolumn{2}{c|}{\textbf{\acrshort{PGD++}}} & \multirow{2}{*}{\textbf{\acrshort{APGD}}} & \textbf{Square} & \multicolumn{2}{c}{\textbf{\acrshort{PGD++}}} \\ 
 &  & \textbf{Attack} & \textbf{\acrshort{NJS}} & \textbf{\acrshort{HNS}} &  & \textbf{Attack} & \textbf{\acrshort{NJS}} & \textbf{\acrshort{HNS}} \\
 \midrule[1pt]
 \acrshort{REF} & \textbf{0.00} & 0.55 & \textbf{0.00} & \textbf{0.00} & 0.79 & 2.25 & \textbf{0.00} & \textbf{0.00} \\  
 \acrshort{BNN-WQ} & \textbf{0.00} & 0.41 & \textbf{0.00} & \textbf{0.00} & 8.23 & 1.98 & \textbf{0.00} & \textbf{0.00} \\  
 \acrshort{BNN-WAQ} & 6.32 & 21.45 & \textbf{0.03} & 0.04  & 0.38 & 16.67 & \textbf{0.01} & 0.02\\  
\bottomrule[1.5pt]
\end{tabular}
\vspace{-1ex}
\caption{\em Adversarial accuracy for \acrshort{REF}, \acrshort{BNN-WQ} and \acrshort{BNN-WAQ} trained on \cifar{-10} using \sresnet{-18}. Both our \acrshort{NJS} and \acrshort{HNS} variants consistently outperform \acrfull{APGD}~\citenew{croce2020reliable} performed using \acrfull{DLR} loss and a gradient free attack namely, Square Attack~\citenew{andriushchenko2020square} under $L_\infty$ bound (8/255). \kartik{fix this table by only keeping vgg16 as resnet18 has been put in the main paper}}
\label{tab:apgd_square}
\vspace{-1ex}
\end{table}

==> tables/fgsm.tex <==
\SKIP{
\begin{table*}[t]
\scriptsize
\centering
\begin{tabular}{l|ccc|ccc|ccc|ccc}
\toprule
\multirow{4}{*}{Methods} & \multicolumn{6}{c|}{CIFAR10} & \multicolumn{6}{c}{CIFAR100} \\ 

  & \multicolumn{3}{c|}{ResNet{-18}} & \multicolumn{3}{c|}{VGG{-16}} & \multicolumn{3}{c|}{ResNet{-18}} & \multicolumn{3}{c}{VGG{-16}} \\ 

\cline{2-13} 
%  & \multicolumn{1}{c}{Orig.} & \multicolumn{1}{c}{HN} & MJSV & \multicolumn{1}{c}{FGSM} & \multicolumn{1}{c}{HN} & MJSV & \multicolumn{1}{c}{Orig.} & \multicolumn{1}{c}{HN} & MJSV & \multicolumn{1}{c}{Orig.} & \multicolumn{1}{c}{HN} & MJSV \\ 
 & \multirow{2}{*}{\acrshort{FGSM}} & \multicolumn{2}{c|}{ \acrshort{FGSM++}} & \multirow{2}{*}{\acrshort{FGSM}} & \multicolumn{2}{c|}{\acrshort{FGSM++}} & \multirow{2}{*}{\acrshort{FGSM}} & \multicolumn{2}{c|}{ \acrshort{FGSM++}} & \multirow{2}{*}{\acrshort{FGSM}} & \multicolumn{2}{c}{\acrshort{FGSM++}} \\


 & & \acrshort{HNS} & \acrshort{NJS} & & \acrshort{HNS} & \acrshort{NJS} &  & \acrshort{HNS} & \acrshort{NJS} &  & \acrshort{HNS} & \acrshort{NJS} \\
 
%  & \acrshort{ORIG.} & \acrshort{HNS} & \acrshort{JSVS-GT} & \acrshort{ORIG.} & \acrshort{HNS} & \acrshort{JSVS-GT} & \acrshort{ORIG.} & \acrshort{HNS} & \acrshort{JSVS-GT} & \acrshort{ORIG.} & \acrshort{HNS} & \acrshort{JSVS-GT} \\
\midrule

\acrshort{REF} & 7.62 & \textbf{5.35} & 5.55 & 11.01 & \textbf{9.66} & 10.04 & 9.06 & \textbf{2.70} & 9.23 & 16.28 & \textbf{9.19} & 17.24 \\
\acrshort{BC} \cite{courbariaux2015binaryconnect} & 11.15 & \textbf{3.61} & 3.77 & 27.38 & 5.04 & \textbf{4.96} & 22.67 & \textbf{2.33} & 9.86 & 11.38 & \textbf{4.00} & 11.02 \\
\acrshort{PQ} \cite{bai2018proxquant} & 52.97 & \textbf{4.24} & 4.50 & 27.46 & 5.43 & \textbf{5.38} & 23.00 & \textbf{3.83} & 13.30 & 9.38 & \textbf{2.68} & 9.40 \\
\acrshort{PMF} \cite{ajanthan2019proximal} & 48.65 & \textbf{3.19} & 3.22 & 54.87 & \textbf{5.15} & 5.19 & 23.11 & \textbf{3.78} & 13.58 & 25.09 & \textbf{5.10} & 15.73 \\
\acrshort{MD}-$\tanh$-\acrshort{S} \cite{ajanthan2019mirror} & 40.49 & \textbf{2.51} & 3.46 & 57.55 & \textbf{3.43} & 4.00 & 25.22 & \textbf{1.80} & 14.08 & 19.82 & \textbf{1.76} & 7.98 \\
\acrshort{BNN-WAQ} \cite{hubara2016binarized} & 40.84 & \textbf{19.09} & 19.46 & 79.92 & \textbf{15.39} & 15.96 & - & - & - & - & - & - \\
\bottomrule
\end{tabular}
\vspace{1ex}

\caption{\em Adversarial accuracy on the test set for binary neural networks using different methods for quantization using original \acrshort{FGSM} attack and \acrshort{FGSM++} attack with \acrshort{NJS} and \acrshort{HNS}.
}
\label{tab:mfgsm}
\end{table*}
}





\begin{table*}[t]
\scriptsize
\centering
\begin{tabular}{l|ccc|ccc|ccc|ccc}
\toprule
\multirow{4}{*}{Methods} & \multicolumn{6}{c|}{CIFAR10} & \multicolumn{6}{c}{CIFAR100} \\ 

  & \multicolumn{3}{c|}{ResNet{-18}} & \multicolumn{3}{c|}{VGG{-16}} & \multicolumn{3}{c|}{ResNet{-18}} & \multicolumn{3}{c}{VGG{-16}} \\ 

\cline{2-13} 
%  & \multicolumn{1}{c}{Orig.} & \multicolumn{1}{c}{HN} & MJSV & \multicolumn{1}{c}{FGSM} & \multicolumn{1}{c}{HN} & MJSV & \multicolumn{1}{c}{Orig.} & \multicolumn{1}{c}{HN} & MJSV & \multicolumn{1}{c}{Orig.} & \multicolumn{1}{c}{HN} & MJSV \\ 
 & \multirow{2}{*}{\acrshort{FGSM}} & \multicolumn{2}{c|}{ \acrshort{FGSM++}} & \multirow{2}{*}{\acrshort{FGSM}} & \multicolumn{2}{c|}{\acrshort{FGSM++}} & \multirow{2}{*}{\acrshort{FGSM}} & \multicolumn{2}{c|}{ \acrshort{FGSM++}} & \multirow{2}{*}{\acrshort{FGSM}} & \multicolumn{2}{c}{\acrshort{FGSM++}} \\


 & & \acrshort{HNS} & \acrshort{NJS} & & \acrshort{HNS} & \acrshort{NJS} &  & \acrshort{HNS} & \acrshort{NJS} &  & \acrshort{HNS} & \acrshort{NJS} \\
 
%  & \acrshort{ORIG.} & \acrshort{HNS} & \acrshort{JSVS-GT} & \acrshort{ORIG.} & \acrshort{HNS} & \acrshort{JSVS-GT} & \acrshort{ORIG.} & \acrshort{HNS} & \acrshort{JSVS-GT} & \acrshort{ORIG.} & \acrshort{HNS} & \acrshort{JSVS-GT} \\
\midrule

\acrshort{REF} & 7.62 & \textbf{5.35} & 5.55 & 11.01 & \textbf{9.66} & 10.04 & 9.06 & \textbf{2.70} & 9.23 & 16.28 & \textbf{9.19} & 17.24 \\
% \acrshort{BC} \cite{courbariaux2015binaryconnect} & 11.15 & \textbf{3.61} & 3.77 & 27.38 & 5.04 & \textbf{4.96} & 22.67 & \textbf{2.33} & 9.86 & 11.38 & \textbf{4.00} & 11.02 \\
% \acrshort{PQ} \cite{bai2018proxquant} & 52.97 & \textbf{4.24} & 4.50 & 27.46 & 5.43 & \textbf{5.38} & 23.00 & \textbf{3.83} & 13.30 & 9.38 & \textbf{2.68} & 9.40 \\
% \acrshort{PMF} \cite{ajanthan2019proximal} & 48.65 & \textbf{3.19} & 3.22 & 54.87 & \textbf{5.15} & 5.19 & 23.11 & \textbf{3.78} & 13.58 & 25.09 & \textbf{5.10} & 15.73 \\
\acrshort{BWN} & 40.49 & \textbf{2.51} & 3.46 & 57.55 & \textbf{3.43} & 4.00 & 25.22 & \textbf{1.80} & 14.08 & 19.82 & \textbf{1.76} & 7.98 \\
\acrshort{BNN-WAQ} & 40.84 & \textbf{19.09} & 19.46 & 79.92 & \textbf{15.39} & 15.96 & - & - & - & - & - & - \\
\bottomrule
\end{tabular}
\vspace{1ex}

\caption{\em Adversarial accuracy on the test set for binary neural networks using different methods for quantization using original \acrshort{FGSM} attack and \acrshort{FGSM++} attack with \acrshort{NJS} and \acrshort{HNS} \kartik{change caption}.
}
\label{tab:mfgsm}
\end{table*}


%%%%%%%%%%%%%

% \begin{table*}[!t]
% \centering
% % \vspace{0mm}
% % \begin{center}
% \scriptsize

% \begin{tabular}{ccccc}
% \centering
% \begin{tabular}{l|ccc|ccc}
% \toprule

% \multirow{4}{*}{Methods} & \multicolumn{6}{c}{CIFAR10} \\ 

%   & \multicolumn{3}{c|}{ResNet{-18}} & \multicolumn{3}{c}{VGG{-16}} \\ 

% \cline{2-7} 
%  & \multirow{2}{*}{\acrshort{FGSM}} & \multicolumn{2}{c|}{ \acrshort{FGSM++}} & \multirow{2}{*}{\acrshort{FGSM}} & \multicolumn{2}{c}{\acrshort{FGSM++}} \\


%  & & \acrshort{HNS} & \acrshort{NJS} & & \acrshort{HNS} & \acrshort{NJS} \\
 
% \midrule

% \acrshort{REF} & 7.62 & 5.35 & 5.55 & 11.01 & 9.66 & 10.04 \\
% \acrshort{BC} \cite{courbariaux2015binaryconnect} & 11.15 & 3.61 & 3.77 & 27.38 & 5.04 & 4.96 \\
% \acrshort{PQ} \cite{bai2018proxquant} & 52.97 & 4.24 & 4.50 & 27.46 & 5.43 & 5.38 \\
% \acrshort{PMF} \cite{ajanthan2019proximal} & 48.65 & 3.19 & 3.22 & 54.87 & 5.15 & 5.19 \\
% \acrshort{MD}-$\tanh$-\acrshort{S} \cite{ajanthan2019mirror} & 40.49 & 2.51 & 3.46 & 57.55 & 3.43 & 4.00 \\
% \acrshort{BNN-WAQ} \cite{hubara2016binarized} & 40.84 & 19.09 & 19.46 & 79.92 & 15.39 & 15.96 \\
% \bottomrule
% \end{tabular}
% &
% &
% &
% \begin{tabular}{l|ccc|ccc}
% \toprule

% \multirow{4}{*}{Methods} & \multicolumn{6}{c}{CIFAR100} \\ 

%   & \multicolumn{3}{c|}{ResNet{-18}} & \multicolumn{3}{c}{VGG{-16}} \\ 

% \cline{2-7} 
%  & \multirow{2}{*}{\acrshort{FGSM}} & \multicolumn{2}{c|}{ \acrshort{FGSM++}} & \multirow{2}{*}{\acrshort{FGSM}} & \multicolumn{2}{c}{\acrshort{FGSM++}} \\


%  & & \acrshort{HNS} & \acrshort{NJS} & & \acrshort{HNS} & \acrshort{NJS} \\
 
% \midrule

% \acrshort{REF} & 9.06 &  & 9.23 & 16.28 & 0.32 & 17.24 \\
% \acrshort{BC} \cite{courbariaux2015binaryconnect} & 22.67 &  & 9.86 & 11.38 &  & 11.02 \\
% \acrshort{PQ} \cite{bai2018proxquant}  & 23.00 &  & 13.30 & 9.38 & 0.03 & 9.40 \\
% \acrshort{PMF} \cite{ajanthan2019proximal} & 23.11 &  & 13.58 & 25.09 & 0.43 & 15.73 \\
% \acrshort{MD}-$\tanh$-\acrshort{S} \cite{ajanthan2019mirror} & 25.22 &  & 14.08 & 19.82 &  & 7.98 \\
% % \acrshort{BNN-WAQ} \cite{hubara2016binarized} & 40.84 & 19.09 & 19.46 & 79.92 & 15.39 & 15.96 \\
% \bottomrule
% \end{tabular}
% % \hspace{7mm}
% % \raisebox{6\height}{\bmvaHangBox{\includegraphics[width=4cm]{figures/ransacvscullnet.pdf}}}\\
% \\
% % \vspace{1mm}

% \it (a) & 
% % \vspace{1mm}
% &
%     &
% \it (b) 
% \end{tabular}\\
% % \end{center}
% \vspace{1mm}

% \caption{\em Adversarial accuracy on the test set for binary neural networks using different methods for quantization using Original \acrshort{FGSM} attack and \acrshort{FGSM++} attack with \acrshort{NJS} and \acrshort{HNS}.
% }
% \label{tab:mfgsm}

% % \vspace{-5mm}
% \end{table*}



% \begin{table}[t]
% \scriptsize
% \centering
% \begin{tabular}{l|ccc|ccc|ccc|ccc}
% \toprule
% \multirow{4}{*}{Methods} & \multicolumn{6}{c|}{CIFAR10} & \multicolumn{6}{c}{CIFAR100} \\ 

%   & \multicolumn{3}{c|}{ResNet{-18}} & \multicolumn{3}{c|}{VGG{-16}} & \multicolumn{3}{c|}{ResNet{-18}} & \multicolumn{3}{c}{VGG{-16}} \\ 

% \cline{2-13} 
% %  & \multicolumn{1}{c}{Orig.} & \multicolumn{1}{c}{HN} & MJSV & \multicolumn{1}{c}{FGSM} & \multicolumn{1}{c}{HN} & MJSV & \multicolumn{1}{c}{Orig.} & \multicolumn{1}{c}{HN} & MJSV & \multicolumn{1}{c}{Orig.} & \multicolumn{1}{c}{HN} & MJSV \\ 
%  & \multirow{2}{*}{\acrshort{FGSM}} & \multicolumn{2}{c|}{ \acrshort{FGSM++}} & \multirow{2}{*}{\acrshort{FGSM}} & \multicolumn{2}{c|}{\acrshort{FGSM++}} & \multirow{2}{*}{\acrshort{FGSM}} & \multicolumn{2}{c|}{ \acrshort{FGSM++}} & \multirow{2}{*}{\acrshort{FGSM}} & \multicolumn{2}{c}{\acrshort{FGSM++}} \\


%  & & \acrshort{HNS} & \acrshort{NJS} & & \acrshort{HNS} & \acrshort{NJS} &  & \acrshort{HNS} & \acrshort{NJS} &  & \acrshort{HNS} & \acrshort{NJS} \\
 
% %  & \acrshort{ORIG.} & \acrshort{HNS} & \acrshort{JSVS-GT} & \acrshort{ORIG.} & \acrshort{HNS} & \acrshort{JSVS-GT} & \acrshort{ORIG.} & \acrshort{HNS} & \acrshort{JSVS-GT} & \acrshort{ORIG.} & \acrshort{HNS} & \acrshort{JSVS-GT} \\
% \midrule

% \acrshort{REF} & 7.62 & 5.35 & 5.55 & 11.01 & 9.66 & 10.04 & 9.06 &  & 9.23 & 16.28 & 0.32 & 17.24 \\
% \acrshort{BC} \cite{courbariaux2015binaryconnect} & 11.15 & 3.61 & 3.77 & 27.38 & 5.04 & 4.96 & 22.67 &  & 9.86 & 11.38 &  & 11.02 \\
% \acrshort{PQ} \cite{bai2018proxquant} & 52.97 & 4.24 & 4.50 & 27.46 & 5.43 & 5.38 & 23.00 &  & 13.30 & 9.38 & 0.03 & 9.40 \\
% \acrshort{PMF} \cite{ajanthan2019proximal} & 48.65 & 3.19 & 3.22 & 54.87 & 5.15 & 5.19 & 23.11 &  & 13.58 & 25.09 & 0.43 & 15.73 \\
% \acrshort{MD}-$\tanh$-\acrshort{S} \cite{ajanthan2019mirror} & 40.49 & 2.51 & 3.46 & 57.55 & 3.43 & 4.00 & 25.22 &  & 14.08 & 19.82 &  & 7.98 \\
% \acrshort{BNN-WAQ} \cite{hubara2016binarized} & 40.84 & 19.09 & 19.46 & 79.92 & 15.39 & 15.96 &  &  &  &  &  & \\
% \bottomrule
% \end{tabular}
% \vspace{1ex}

% \caption{\em Adversarial accuracy on the test set for binary neural networks using different methods for quantization using Original \acrshort{FGSM} attack and \acrshort{FGSM++} attack with \acrshort{NJS} and \acrshort{HNS}.
% }
% \label{tab:mfgsm}

% \end{table}




==> tables/pgd_l2.tex <==
\SKIP{
\begin{table*}[t]
\scriptsize
\centering
\begin{tabular}{l|ccc|ccc|ccc|ccc}
\toprule
\multirow{3}{*}{Methods} & \multicolumn{6}{c|}{CIFAR10} & \multicolumn{6}{c}{CIFAR100} \\ 

  & \multicolumn{3}{c|}{ResNet{-18}} & \multicolumn{3}{c|}{VGG{-16}} & \multicolumn{3}{c|}{ResNet{-18}} & \multicolumn{3}{c}{VGG{-16}} \\ 

\cline{2-13} 
%  & \multicolumn{1}{c}{Orig.} & \multicolumn{1}{c}{HN} & MJSV & \multicolumn{1}{c}{PGD} & \multicolumn{1}{c}{HN} & MJSV & \multicolumn{1}{c}{Orig.} & \multicolumn{1}{c}{HN} & MJSV & \multicolumn{1}{c}{Orig.} & \multicolumn{1}{c}{HN} & MJSV \\ 
 & \multirow{2}{*}{\acrshort{PGD}} & \multicolumn{2}{c|}{ \acrshort{PGD++}} & \multirow{2}{*}{\acrshort{PGD}} & \multicolumn{2}{c|}{\acrshort{PGD++}} & \multirow{2}{*}{\acrshort{PGD}} & \multicolumn{2}{c|}{ \acrshort{PGD++}} & \multirow{2}{*}{\acrshort{PGD}} & \multicolumn{2}{c}{\acrshort{PGD++}} \\


 & & \acrshort{HNS} & \acrshort{NJS} & & \acrshort{HNS} & \acrshort{NJS} &  & \acrshort{HNS} & \acrshort{NJS} &  & \acrshort{HNS} & \acrshort{NJS} \\
 \midrule

\acrshort{REF} & 45.18 & \textbf{0.05} & 0.09 & 2.23 & 1.10 & \textbf{0.78} & 5.38 & \textbf{0.15} & 0.17 & 4.87 & \textbf{1.38} & 1.50 \\
\acrshort{BC} \cite{courbariaux2015binaryconnect} & 61.11 & 0.24 & \textbf{0.18} & 46.24 & \textbf{1.58} & 1.63 & 28.98 & \textbf{0.38} & 5.27 & 6.78 & \textbf{0.58} & 4.66 \\
\acrshort{PQ} \cite{bai2018proxquant} & 69.57 & 0.50 & \textbf{0.35} & 27.33 & \textbf{1.72} & 2.25 & 29.57 & \textbf{1.24} & 9.21 & 5.05 & \textbf{0.75} & 5.10 \\
\acrshort{PMF} \cite{ajanthan2019proximal} & 74.72 & 0.04 & \textbf{0.02} & 55.82 & 2.85 & \textbf{2.71} & 45.97 & \textbf{0.71} & 6.60  & 30.91 & \textbf{1.61} & 8.62 \\
\acrshort{MD}-$\tanh$-\acrshort{S} \cite{ajanthan2019mirror} & 74.59 & 0.06 & \textbf{0.05} & 61.90 & 3.18  & \textbf{0.35} & 42.67 & \textbf{0.26} & 6.79 & 19.26 & \textbf{0.63} & 3.17 \\
\acrshort{BNN-WAQ} \cite{hubara2016binarized} & 67.84 & 2.59 & \textbf{2.33} & 85.62 & 0.62 & \textbf{0.49} & - & - & - & - & - & - \\
\bottomrule
\end{tabular}
\vspace{1ex}

\caption{\em Adversarial accuracy on the test set for binary neural networks using different methods for quantization using original $L_2$ bounded \acrshort{PGD} attack and \acrshort{PGD++} attack with \acrshort{NJS} and \acrshort{HNS}.
}
\label{tab:mpgdl2}
\end{table*}
}



\begin{table*}[t]
\scriptsize
\centering
\begin{tabular}{l|ccc|ccc|ccc|ccc}
\toprule
\multirow{3}{*}{Methods} & \multicolumn{6}{c|}{CIFAR10} & \multicolumn{6}{c}{CIFAR100} \\ 

  & \multicolumn{3}{c|}{ResNet{-18}} & \multicolumn{3}{c|}{VGG{-16}} & \multicolumn{3}{c|}{ResNet{-18}} & \multicolumn{3}{c}{VGG{-16}} \\ 

\cline{2-13} 
%  & \multicolumn{1}{c}{Orig.} & \multicolumn{1}{c}{HN} & MJSV & \multicolumn{1}{c}{PGD} & \multicolumn{1}{c}{HN} & MJSV & \multicolumn{1}{c}{Orig.} & \multicolumn{1}{c}{HN} & MJSV & \multicolumn{1}{c}{Orig.} & \multicolumn{1}{c}{HN} & MJSV \\ 
 & \multirow{2}{*}{\acrshort{PGD}} & \multicolumn{2}{c|}{ \acrshort{PGD++}} & \multirow{2}{*}{\acrshort{PGD}} & \multicolumn{2}{c|}{\acrshort{PGD++}} & \multirow{2}{*}{\acrshort{PGD}} & \multicolumn{2}{c|}{ \acrshort{PGD++}} & \multirow{2}{*}{\acrshort{PGD}} & \multicolumn{2}{c}{\acrshort{PGD++}} \\


 & & \acrshort{HNS} & \acrshort{NJS} & & \acrshort{HNS} & \acrshort{NJS} &  & \acrshort{HNS} & \acrshort{NJS} &  & \acrshort{HNS} & \acrshort{NJS} \\
 \midrule

\acrshort{REF} & 45.18 & \textbf{0.05} & 0.09 & 2.23 & 1.10 & \textbf{0.78} & 5.38 & \textbf{0.15} & 0.17 & 4.87 & \textbf{1.38} & 1.50 \\
% \acrshort{BC} \cite{courbariaux2015binaryconnect} & 61.11 & 0.24 & \textbf{0.18} & 46.24 & \textbf{1.58} & 1.63 & 28.98 & \textbf{0.38} & 5.27 & 6.78 & \textbf{0.58} & 4.66 \\
% \acrshort{PQ} \cite{bai2018proxquant} & 69.57 & 0.50 & \textbf{0.35} & 27.33 & \textbf{1.72} & 2.25 & 29.57 & \textbf{1.24} & 9.21 & 5.05 & \textbf{0.75} & 5.10 \\
% \acrshort{PMF} \cite{ajanthan2019proximal} & 74.72 & 0.04 & \textbf{0.02} & 55.82 & 2.85 & \textbf{2.71} & 45.97 & \textbf{0.71} & 6.60  & 30.91 & \textbf{1.61} & 8.62 \\
\acrshort{BWN} & 74.59 & 0.06 & \textbf{0.05} & 61.90 & 3.18  & \textbf{0.35} & 42.67 & \textbf{0.26} & 6.79 & 19.26 & \textbf{0.63} & 3.17 \\
\acrshort{BNN-WAQ} & 67.84 & 2.59 & \textbf{2.33} & 85.62 & 0.62 & \textbf{0.49} & - & - & - & - & - & - \\
\bottomrule
\end{tabular}
\vspace{1ex}

\caption{\em Adversarial accuracy on the test set for binary neural networks using different methods for quantization using original $L_2$ bounded \acrshort{PGD} attack and \acrshort{PGD++} attack with \acrshort{NJS} and \acrshort{HNS}. \kartik{change caption}
}
\label{tab:mpgdl2}
\end{table*}

==> tables/pgd_linf.tex <==
\begin{table*}[t]
\centering
\scriptsize
\begin{tabular}{l|ccc|ccc|ccc|ccc}
\toprule
\multirow{3}{*}{Methods} & \multicolumn{6}{c|}{CIFAR10} & \multicolumn{6}{c}{CIFAR100} \\ 

  & \multicolumn{3}{c|}{ResNet{-18}} & \multicolumn{3}{c|}{VGG{-16}} & \multicolumn{3}{c|}{ResNet{-18}} & \multicolumn{3}{c}{VGG{-16}} \\ 

\cline{2-13} 
%  & \multicolumn{1}{c}{Orig.} & \multicolumn{1}{c}{HN} & MJSV & \multicolumn{1}{c}{PGD} & \multicolumn{1}{c}{HN} & MJSV & \multicolumn{1}{c}{Orig.} & \multicolumn{1}{c}{HN} & MJSV & \multicolumn{1}{c}{Orig.} & \multicolumn{1}{c}{HN} & MJSV \\ 
 & \multirow{2}{*}{\acrshort{PGD}} & \multicolumn{2}{c|}{ \acrshort{PGD++}} & \multirow{2}{*}{\acrshort{PGD}} & \multicolumn{2}{c|}{\acrshort{PGD++}} & \multirow{2}{*}{\acrshort{PGD}} & \multicolumn{2}{c|}{ \acrshort{PGD++}} & \multirow{2}{*}{\acrshort{PGD}} & \multicolumn{2}{c}{\acrshort{PGD++}} \\


 & & \acrshort{HNS} & \acrshort{NJS} & & \acrshort{HNS} & \acrshort{NJS} &  & \acrshort{HNS} & \acrshort{NJS} &  & \acrshort{HNS} & \acrshort{NJS} \\
 \midrule

\acrshort{REF} & 0.00 & 0.00 & 0.00 & 0.04 & 0.00 & 0.00 & 0.14 & \textbf{0.00} & 0.14 & 1.53 & \textbf{0.25} & 0.95 \\
% \acrshort{BC} \cite{courbariaux2015binaryconnect} & 4.40 & \textbf{0.00} & \textbf{0.00} & 9.28 & \textbf{0.36} & 0.37 & 3.60 & \textbf{0.00} & 1.33 & 1.84 & \textbf{0.04} & 1.57 \\
% \acrshort{PQ} \cite{bai2018proxquant} & 22.49 & \textbf{0.01} & \textbf{0.01} & 23.41 & \textbf{0.00} & \textbf{0.00} & 4.80 & \textbf{0.23} & 3.09 & 1.41 & \textbf{0.14} & 1.39 \\
% \acrshort{PMF} \cite{ajanthan2019proximal} & 33.02 & \textbf{0.00} & \textbf{0.00} & 54.11 & \textbf{0.00} & \textbf{0.00} & 6.22 & \textbf{0.05} & 2.11 & 8.34 & \textbf{0.21} & 3.06 \\
\acrshort{BWN} & 26.98 & \textbf{0.00} & \textbf{0.00} & 47.32 & 0.02 & \textbf{0.00} & 8.23 & \textbf{0.00} & 2.45 & 17.44 & \textbf{0.16} & 0.88 \\
\acrshort{BNN-WAQ}\footnotemark & 8.57 & 0.04 & \textbf{0.03} & 78.01 & 0.02 & \textbf{0.01} & - & - & - & - & - & - \\
\bottomrule
\end{tabular}
\vspace{1ex}

\caption{\em Adversarial accuracy on the test set for binary neural networks using different methods for quantization using original $L_\infty$ bounded \acrshort{PGD} attack and \acrshort{PGD++} attack with \acrshort{NJS} and \acrshort{HNS} \kartik{change caption}.
}
\label{tab:mpgdlinf}
\end{table*}


==> tables/psinorm_jsv_study.tex <==
\SKIP{
\begin{table*}[t]
\scriptsize
\centering
\begin{tabular}{l|ccccccc}
\toprule
Methods & \acrshort{REF} & Adv. Train & \acrshort{BC} \cite{courbariaux2015binaryconnect} & \acrshort{PQ} \cite{bai2018proxquant} & \acrshort{PMF} \cite{ajanthan2019proximal} & \acrshort{MD}-$\tanh$-\acrshort{S} \cite{ajanthan2019mirror} &\acrshort{BNN-WAQ} \cite{hubara2016binarized} \\ 
\midrule
 \acrshort{JSV} (Mean) & $8.09\mathrm{e}{+00}$ & $5.15\mathrm{e}{-01}$ & $1.61\mathrm{e}{+01}$ & $2.34\mathrm{e}{+01}$ & $4.46\mathrm{e}{+01}$ & $3.53\mathrm{e}{+01}$ & $1.11\mathrm{e}{+00}$ \\ 
 \acrshort{JSV} (Std.) & $6.27\mathrm{e}{+00}$ & $4.10\mathrm{e}{-01}$ & $1.88\mathrm{e}{+01}$ & $2.35\mathrm{e}{+01}$ & $1.11\mathrm{e}{+02}$ & $3.53\mathrm{e}{+01}$ & $1.97\mathrm{e}{+00}$ \\
 $\|\psi\|_2$ (Mean) & $9.08\mathrm{e}{-03}$ & $2.33\mathrm{e}{-01}$ & $1.18\mathrm{e}{-02}$ & $6.75\mathrm{e}{-03}$ & $8.50\mathrm{e}{-03}$ & $6.20\mathrm{e}{-03}$ & $9.46\mathrm{e}{-03}$ \\
\bottomrule
\end{tabular}
\vspace{1ex}

\caption{\em Mean and standard deviation of \acrfull{JSV} and mean $\|\psi\|_2$ for different methods on \cifar{-10} with \sresnet{-18} computed with 500 correctly classified samples. Note the norm of the error signal $\psi$ is very small in all cases except for Adv. Train, indicating that all models are over confident (probabilities close to one-hot) except for Adv. Train which is in fact under confident for correctly classified samples.
Furthermore, one can clearly see that \bnns{} (except \acrshort{BNN-WAQ}) have much higher \acrshort{JSV} mean and we believe this leads to gradient vanishing, \ie, increased scale for logits $\rva^K$ and in turn reduced (if not zero) error signal $\psi$.
}
\label{tab:psinorm_jsv_study}
\end{table*}
}

\begin{table*}[t]
\centering
\small
\begin{tabular}{l|cccc}
\toprule[1.5pt]
\textbf{Methods} & \textbf{\acrshort{REF}} & \textbf{Adv. Train} & \textbf{\acrshort{BNN-WQ}}  & \textbf{\acrshort{BNN-WAQ}} \\ 
%  &  &  & \citenew{ajanthan2019mirror} & \citenew{hubara2016binarized} \\ 

\midrule[1pt]
 \textbf{\acrshort{JSV} (Mean)} & $8.09\mathrm{e}{+00}$ & $5.15\mathrm{e}{-01}$ &  $3.53\mathrm{e}{+01}$ & $1.11\mathrm{e}{+00}$ \\ 
 \textbf{\acrshort{JSV} (Std.)} & $6.27\mathrm{e}{+00}$ & $4.10\mathrm{e}{-01}$ & $3.53\mathrm{e}{+01}$ & $1.97\mathrm{e}{+00}$ \\
 \textbf{$\|\psi\|_2$ (Mean)} & $9.08\mathrm{e}{-03}$ & $2.33\mathrm{e}{-01}$ & 
 $6.20\mathrm{e}{-03}$ & $9.46\mathrm{e}{-03}$ \\
\bottomrule[1.5pt]
\end{tabular}
\vspace{1ex}

\caption{\em Mean and standard deviation of \acrfull{JSV} and mean $\|\psi\|_2$ for different methods on \cifar{-10} with \sresnet{-18} computed with 500 correctly classified samples. Note, the norm of the error signal $\psi$ is very small in all cases except for Adv. Train, indicating that all models are over confident (probabilities close to one-hot) except for Adv. Train which is in fact under confident for correctly classified samples. Furthermore, one can clearly see that \acrshort{BNN-WQ} have much higher \acrshort{JSV} mean and we believe this leads to gradient vanishing, \ie, increased scale for logits $\rva^K$ and in turn reduced (if not zero) error signal $\psi$.\kartik{not sure about last line; maybe need to move this to appendix}}
\label{tab:psinorm_jsv_study}
\end{table*}



\SKIP{
\begin{table}[t]
%\begin{wrapfigure}{r}{0.6\textwidth}
%\begin{figure}
\vspace{-1ex}
%\small
\begin{minipage}[c]{0.5\linewidth}
    \centering    
\begin{tabular}{l|cccc}
\toprule[1.5pt]
\textbf{Methods} & \textbf{\acrshort{REF}} & \textbf{Adv. Train} & \textbf{\acrshort{BNN-WQ}}  & \textbf{\acrshort{BNN-WAQ}} \\ 
%  &  &  & \citenew{ajanthan2019mirror} & \citenew{hubara2016binarized} \\ 

\midrule[1pt]
 \textbf{\acrshort{JSV} (Mean)} & $8.09\mathrm{e}{+00}$ & $5.15\mathrm{e}{-01}$ &  $3.53\mathrm{e}{+01}$ & $1.11\mathrm{e}{+00}$ \\ 
 \textbf{\acrshort{JSV} (Std.)} & $6.27\mathrm{e}{+00}$ & $4.10\mathrm{e}{-01}$ & $3.53\mathrm{e}{+01}$ & $1.97\mathrm{e}{+00}$ \\
 \textbf{$\|\psi\|_2$ (Mean)} & $9.08\mathrm{e}{-03}$ & $2.33\mathrm{e}{-01}$ & 
 $6.20\mathrm{e}{-03}$ & $9.46\mathrm{e}{-03}$ \\
\bottomrule[1.5pt]
\end{tabular}

\end{minipage}\hfill
\begin{minipage}[c]{0.5\linewidth}
    \vspace{-1ex}
\caption{\em Mean and standard deviation of \acrfull{JSV} and mean $\|\psi\|_2$ for different methods on \cifar{-10} with \sresnet{-18} computed with 500 correctly classified samples. Note, the norm of the error signal $\psi$ is very small in all cases except for Adv. Train, indicating that all models are over confident (probabilities close to one-hot) except for Adv. Train which is in fact under confident for correctly classified samples. Furthermore, one can clearly see that \acrshort{BNN-WQ} have much higher \acrshort{JSV} mean and we believe this leads to gradient vanishing, \ie, increased scale for logits $\rva^K$ and in turn reduced (if not zero) error signal $\psi$.\kartik{not sure about last line}}
\label{tab:psinorm_jsv_study}
    \end{minipage}
\end{table}
}

==> tables/rho_vs_fgsm++.tex <==
\begin{table}[h]
% \scriptsize
\centering
\begin{tabular}{l|c|c|c|c|c|c}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{6}{c}{\acrshort{FGSM++}}\\
& $\rho=1e-30$ & $\rho=1e-20$ & $\rho=1e-05$ & $\rho=1e-01$ & $\rho=2e-01$ & $\rho=5e-01$ \\
\midrule
\acrshort{REF} & 23.95 & 23.78 & \textbf{20.46} & 23.10 & 23.47 & 23.92 \\
\acrshort{REF}$^*$ & 75.92 & \textbf{75.88} & 76.25 & 77.61 & 77.87 & 78.37 \\
\acrshort{MD}-$\tanh$-\acrshort{S} & 54.31 & 53.35 & \textbf{24.52} & 28.60 & 29.35 & 30.34 \\
\acrshort{MD}-$\tanh$-\acrshort{S}$^*$ & 70.02 & \textbf{69.98} & 70.34 & 71.67 & 72.04 & 72.91 \\
\acrshort{GD}-$\tanh$ & 60.85 & 58.37 & \textbf{21.80} & 26.12 & 26.93 & 28.42 \\
\acrshort{GD}-$\tanh^*$ & 70.34 & \textbf{70.33} & 70.74 & 72.05 & 72.41 & 73.15 \\
\bottomrule
\end{tabular}
\vspace{1ex}

\caption{\em Adversarial accuracy on the test set for adversarially trained networks and binary neural networks with different methods for quantization using $L_\infty$ bounded \acrshort{FGSM++} attack with varying $\rho$ as lowerbound on the gradient of network output. Here * denotes the adversarially trained models obtained where adversarial samples are generated using $L_\infty$ bounded \acrshort{PGD} attack with with $T = 7$ iterations, $\eta=2$ and $\epsilon=8$.
}
\label{tab:rho_vs_fgsm++}
\vspace{-6ex}
\end{table}
